Towards Interdependent Safety Security Assessments using Bowties

We present a way to combine security and safety assessments using Bowtie Diagrams. Bowties model both the causes leading up to a central failure event and consequences which arise from that event, as well as barriers which impede events. Bowties have previously been used separately for security and safety assessments, but we suggest that a unified treatment in a single model can elegantly capture safety-security interdependencies of several kinds. We showcase our approach with the example of the October 2021 Facebook DNS shutdown, examining the chains of events and the interplay between the security and safety barriers which caused the outage.

==> texts/background.tex <==
% was: Background (instead of previous work)
\section{Diagrammatic Representations}
\label{sec:background}

% Formal Foundations for Hierarchical Safety Cases
% DA: don't think subsect needed really
% \subsection{Diagrammatic Representations of Events and Relationships}
\renewcommand{\arraystretch}{1.2}
\begin{table}[htb!]
    \centering
        \caption{Symbols and Relationships in a fault tree}
    \begin{tabular}{c|p{0.7\columnwidth}}
    \hline
    \multicolumn{2}{c}{\textbf{Event Types}}\\\hline
     \noalign{\smallskip}
    %   \tikz \draw (2,2) ellipse (10pt and 10pt); & \textit{Initial cause event} - initial fault requiring no further development \\
    %   &\\
    \centering   \begin{tikzpicture}[baseline=0, scale=.4] \draw (0,0) rectangle (2,1); \end{tikzpicture} &   \textit{Intermediate event} - an identity function labelling outgoing edges. \\
    
    \centering   \begin{tikzpicture}[baseline=0] \draw (.2,0.2) ellipse (10pt and 6pt); \end{tikzpicture} {}  &   \textit{Prevention } - restrictive conditions, must fail to progress \vspace{0em}\\
    
     \centering   \begin{tikzpicture} \node [trapezium, trapezium angle=60, minimum width=25, draw]  {};\end{tikzpicture} &   \textit{LEAF} - initiation event (BEs in Fault Trees) eventual outcome (in Event Trees) 
    \\     \hline
   \multicolumn{2}{c}{\textbf{Relationship Types}}\\\hline
          \noalign{\smallskip}
            \begin{minipage}{.06\textwidth}
                     \includegraphics[width=\textwidth]{figs/INHIBIT.pdf}
            \end{minipage}

        & INHIBIT - output occurs if the LH occurs and prevention does not \\ % 
    \resizebox{35pt}{15pt}{%
   \begin{circuitikz} \draw
        (2,3) node[or port, fill=none] (myor) {}
        
        (myor.in 1) node[left =.2cm] (a) { }
        (myor.in 2) node[left =.2cm] (b) { }
        (myor.out)  node[right=.2cm] (c) { }
        
        (myor.in 1) -- (a)
        (myor.in 2) -- (b)
        (myor.out)  -- (c);
        % \addvmargin{1mm}
        \end{circuitikz}}&   OR -  output occurs if at least one of the inputs occurs\\
        \resizebox{35pt}{15pt}{%
   \begin{circuitikz} \draw
        (1.2,2.2) node[and port, fill=none] (myor) {}
        
        (myor.in 1) node[left =.2cm] (a) {}
        (myor.in 2) node[left =.2cm] (b) {}
        (myor.out)  node[right=.2cm] (c) {}
        
        (myor.in 1) -- (a)
        (myor.in 2) -- (b)
        (myor.out)  -- (c);
        \end{circuitikz}} &   AND - output occurs if both of the inputs occur\\
%      \resizebox{50pt}{20pt}{%
%   \begin{circuitikz} \draw
%         (1,2) node[xor port, fill=none] (myor) {}
        
%         (myor.in 1) node[left =.2cm] (a) {}
%         (myor.in 2) node[left =.2cm] (b) {}
%         (myor.out)  node[right=.2cm] (c) {}
        
%         (myor.in 1) -- (a)
%         (myor.in 2) -- (b)
%         (myor.out)  -- (c);
%         \end{circuitikz}} &   XOR - output occurs if exactly one of the inputs occurs\\
        
%      \resizebox{50pt}{20pt}{%
%   \begin{circuitikz} \draw
%         (1,1) node[not port, fill=none] (myor) {}
        
%         (myor.in) node[left =.2cm] (a) {A}
%         (myor.out)  node[right=.2cm] (b) {B}
        
%         (myor.in) -- (a)
%         (myor.out)  -- (b);
%         \end{circuitikz}} &   NOT - negation of a fault/attack\\
         

 \hline
    \end{tabular}

    \label{tab:symbols}
  \end{table}

Our bowtie diagrams use Boolean logic gate notation to show relationships between events tracking the passage of failures from ``inputs'' to ``outputs''.
Boxes containing labels describe intermediate events. 
% The symbols for fault tree and attacks trees are interchangeable.
\paragraph{Faults and attacks in the same diagram.} 
Security analysis
traditionally uses attack trees~\cite{schneier1999attack} whilst Safety analysis makes use of fault trees~\cite{vesely1981fault}. One shows the steps
which an attacker can take to achieve a goal whilst the other shows the events leading to a fault.  
Stoelinga, however, has
recently argued that fault trees and attack trees can be treated uniformly in a single structure~\cite{stoelinga2021marriage}.
Tab.~\ref{tab:symbols} shows the symbols we use, following the Fault
Tree Handbook notation~\cite{vesely1981fault}.  
%% RIGHT?
\paragraph{Barriers and defences treated uniformly.}
We further propose to also treat barriers and defences in the same logic.  To
capture actions or conditions that impede fault conditions arising or
defences in an attack tree, we use an \texttt{INHIBIT} gate drawn as a
hexagon.  The orthogonal side input is the inhibiting condition which
prevents the flow of the fault or prevents the attack.

\paragraph{Safety Security Bowties.}
Now that we have a unified tree notation for attack trees and fault trees, we can use event tree tree notation for consequences as usual.  This stays true to the essence of bowties as previously
defined~\cite{de2016bowtie}.
The focal point of the assessment is the critical risk event (or ``top event'', following fault tree parlance).
To the left of the event are potential causes of the risk and ways to reduce them; this is the \emph{prevention assessment}.
On the right on the other hand we observe the outcomes of the risk event known as the \emph{consequence assessment}.
%whilst in practice several risk events may be analyzed at once, usually a single use focus
% This event usually constitutes the focus of the single bowtie assessment, however in practice multiple risk events could be considered.
% DA: seems obvious
% Several different causes may lead to the same event, and several different outcomes might spawn out of this event.
% The bowtie diagram enables you to trace causality across various different causes and outcomes and to conduct a very thorough risk assessment.
% A natural progression from these same concepts is to look at prevention and recovery, addressing the causes and outcomes respectively.
% A prevention to a cause is the application of a mitigator factor which will reduce the risk. 
% Just like the left hand side showcases a set of disruptions which lead to the risk event, the right shows potential outcomes and responses to this event.
% The right hand side of the bowtie is .
%% AKA: (safety response, security XXX?).

An example unlabelled bowtie diagram is shown in Fig.~\ref{fig:bowtie-genera}.
These diagrams are a Boolean network which are static and capture only logical dependencies: a bowtie itself is not quantitative,
but it is a qualitative model that may be analysed quantitatively by adding additional annotations representing risk assessments.  This has been done by various authors for fault and attack trees, 
for example~\cite{ren2017fault,fila2020exploiting}.  
For simplicity in the rest of this paper, we consider the basic logical interpretation only.

\begin{figure}[htb]
     \centering
     \includegraphics[width=0.7\linewidth]{figs/example-bowtie-leafs.pdf}
     \caption{Generic representation of Bowtie Diagram with causes on the left and outcomes on the right.}
     \label{fig:bowtie-genera}
 \end{figure}
 

 





==> texts/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

% \begin{itemize}
%     \item Refinement still to do
%     \item look at more gates to deal with interdependence
%     \item generalise the approach into an algorithms
%     \item need larger scenario to showcase the methodology
%     \end{itemize}

This work presented the first formalisation of safety security interdependence covering the full spectrum of dependencies through the use of bowtie diagrams.
We notice some interesting outcomes: 1) for some of the dependencies dynamic gates are necessary i.e. \texttt{INHIBIT} gates (not typically used).
2) some dependencies make more sense on the outcome of the tree, are beyond the attack/fault tree, and need to be reflected in the recovery phase (showcasing the suitability of bowties as a way to explore interdependence).
We also provide the first formalisation of DPTs alongside its semantics.
Finally, this work is the first to provide formalisations of the safety security interdependence operations under a unified assessment.

\subsection{Related work}
\input{texts/related-work}


\subsection{Next steps}

In order to fully generalise this approach a larger case study should be adapted, in particular further analysis on how the two types of trees, event and disruption, can be chained to combine the analysis of several consequent risk events is desirable.
We also see as desirable the investigation of further gate types to fully encapsulate the the full spectrum of analysis currently seen across the literature.
The formal definition of joining operations we have provided for security and safety assessments presents a unique potential for automating the process of combining safety security analysis, future work into this area would have tremendous impact to more rigorously examine scenarios such as the Facebook DNS incident from both assessment angles.
However there is also a need for further investigation into properties of these provided join operations.
We also see the usefulness of hierarchicalisation as means to combine sequences of events into a single more readable structure.
This has been explored in the past successfully for assurance cases~\cite{denney2015formal} and as in this approach several assessments are joined together under the same formalism, an enhancement of this approach could be even more effective and desirable. 
% Although we note further generalisations may be required as discussed in Sec.~\ref{sec:operations}.
We note that further to the formalisation of the structures and their semantics some distinctions exist in how the probabilities of risk are calculated, however this is orthogonal to the work presented here and we reserve this investigation to future work.




%% DA: not strictly needed at this stage but giving credits helps to steer referees (e.g. away from Ewen!)
\paragraph{Acknowledgements.}  We're grateful to Ewen~Denney for
suggesting to us to investigate bowtie diagrams for safety-security
assessments, as well as comments on an early draft.
This work was funded by the AISEC grant under EPSRC number EP/T027037/1


==> texts/formalisation.tex <==
\section{Formalisation of Safety-Security Bowties}
\label{sec:formalisation}

Like typical bowties a safety-security bowtie will be composed of a \textit{prevention assessment} and a \textit{consequence assessment}.
%
For the prevention assessment we use a \emph{disruption prevention tree} which captures safety and security assessments, as well as 
attack and fault mitigations, which correspond to barriers in traditional bowties~\cite{de2016bowtie}.
%
For the consequence assessment we use an event tree to show the consequences of the risk event and potential outcomes. 
%% DA which is what?
The graphical representation from the figures includes intermediate events between gates, for enhanced understanding, but these are not part of the formalisation.
We first showcase a general structure for trees we make use of for all subsequent formalisations in Sec.~\ref{sec:structure-tree}.
We note that although, we are mostly concerned with trees, we adopt Directed Acyclic Graphs (DAGs) to allow input and outputs to be shared between gates.


\subsection{Structure trees}
\label{sec:structure-tree}
Our models are based on generalised n-ary trees with additional
structure given by a node type labeling. 

%% DA: could put LEAF label here but seems marginally cleaner to not.
\begin{definition}[Structure Tree]
\label{def:st}
A Structure Tree is a tuple $T = \langle N,\mathbb{T},t,\ch\rangle$ where:
\begin{itemize}
    \item $N$ is a finite set of nodes and $\mathbb{T}$ is a set of node types;
    \item $t: N \rightarrow \mathbb{T}$ gives the type of each node;
    \item $\ch: N \rightarrow N^*$ gives the sequence of children of a node.
\end{itemize}
Moreover, T satisfies the following constraints:
\begin{itemize}
    \item $(N,E)$ is a connected DAG where $E = \theset{(v,u) \in N^2 \;|\; u\in \ch(v)}$
    \item $T$ has a unique root, denoted by $R_T:\exists ! R_T \in N . \forall v \in N. R_T \not\in\ch(v)$ (where $\exists !$ stands for unique existence).

\end{itemize}
\end{definition}

Given a type $\LEAFt\in\mathbb{T}$, we write $\leavesof{T} = \theset{v\in N \;|\; t(v)=\LEAFt}$
for the nodes labelled with that type, and similarly for other types.
% We write $\choices{T} = \theset{v\in N \;|\; t(v)=\CHOOSEt}$ for 
% the choice nodes of a DCT $T$.




\subsection{Disruption Trees}

% A recent development in the assessment of safety and security risk has shown that both fault and attack trees,
The notion of Disruption Trees (DTs) is introduced by Stoelinga as the
uniform representation of static safety and security risk models~\cite{stoelinga2021marriage,budde2021attack}.
Although extensions exists to each of these assessments which do result in key differences, in the simplest setting with only \texttt{OR} and \texttt{AND} nodes, they coincide.\footnote{There are subtleties in different
  ways to treat \texttt{OR} gates with quantified safety or security risks, which will not be considered here.}
% Following the formalisation by Stoelinga et al.~\cite{stoelinga2021marriage}.
% A Disruption Tree (DT) is a rooted Directed Acyclic Graph (DAG) with typed nodes representing different gates or leaves.
% % The edges of a
% % DT are given by a function $ch$ that assigns to each node its (possibly empty) sequence of children.,  the empty sequence is denoted by $\epsilon$.
% % DA: this is in the def
% Mostly we are concerned with trees, but DAGS generalise to allow
% input and outputs to be shared between gates.
Following Def.~\ref{def:st} we can interpret Stoelinga's DTs as:

\begin{definition}[Disruption Tree \cite{stoelinga2021marriage}]
  \label{def:dt2}
  A Disruption Tree is a structure tree according to Def.~\ref{def:st} with %
  $\mathbb{T} = \theset{\LEAFt,\ANDt,\ORt}$
  and such that $t(v)=\LEAFt$ if{}f $v\in\leavesof{T}$.
\end{definition}

Semantics pin down the mathematical meaning of models. The basic semantics of a disruption tree is given
by its \emph{structure function} over Booleans $\mathbb{B} = \{1, 0\}$, which defines a function
from leaf events to the root in the obvious way.  
Structure Trees are more lax compared to models we usually want.
 Besides allowing useful DAG structure they include redundancies like
nodes with repeated children.  This is alright for \texttt{AND} and \texttt{OR} but
 would be confusing later on with gates that have some inputs (or
 outputs) being negated (or mutually exclusive).  
We call a
 structure tree (and later variants) \emph{proper} if every child of a
 node is distinct, i.e.,
 $|\theset{\ch(v)\;|\;v\in N}|=\mathit{length}(\ch(v))$.
% %
 From now on we will restrict to models built on proper structure trees.

\subsection{Prevention Assessments}
\label{sec:left}

% \begin{itemize}
%     \item analysis on causes
%     \item discuss generic left hand side of bowtie
%     \item explain the observation that fault tree and attack tree are the same
%     \item differentiate in the OR and explain how we ignore this difference for this particular analysis
%     \item analysis on barriers
%     \item discuss defences and their impacts
%     \item relate to previous work on barriers
%     \item explain defences in terms of inhibit node (match to the semantics)
% \end{itemize}



% \subsubsection{Probability of Failure}

% The probabilities of the initial event taking place is a factor of the different cut sets.
% For any $P(A \wedge B) = P(A) * P(B)$, for any $P(A \vee B)= P(A) + P(B) - P(A \wedge B)$, for any $P(A \veebar B) = P(A) + P(B) - 2*P(A \wedge B)$ and for any $P(A \bhexagon B) = P(A) * P(\neg B)$.
% This can deductively give you the final probability of the failure taking place by traversing the tree.

We turn a Disruption Tree
% DA: already defined above  ~\cite{stoelinga2021marriage,budde2021attack}
into a Disruption Prevention Tree by adding a new gate type for \texttt{INHIBIT}.
% Matching the rest of the DT structure 1-to-1. 
%%% ADD specific definitions

\begin{definition}[Disruption Prevention Tree]
  \label{def:def-dpt}
  A Disruption Prevention Tree (DPT) is a Disruption Tree
  % according to Def.~\ref{def:dt2}
  with an additional binary node type
  $\INHIBITt$, i.e.,
  $\mathbb{T} = \theset{\LEAFt,\ANDt,\ORt,\INHIBITt}$ and
  $|\ch(v)|=2$ whenever $t(v)=\INHIBITt$.  The second child of
  an \INHIBITt node corresponds to
  the inhibiting (prevention) condition.
\end{definition}  
% These labels are $\mathbb{L}=\{\text{\texttt{p,o}}\}$

There is a similarity between Disruption Prevention Trees and Attack-Defence Trees. 
Formalisations of Attack-Defence Trees (see~\cite{kordy2010foundations} for example) label nodes to represent their role in the model as a proponent
(mitigating an attack or protecting against a fault event) or an opponent (actors causing damage leading to the root fault).
It seems possible %% CHECK IT!  
to recover this labelling from the root of DPT flipping the role when consider the prevention
input of \texttt{INHIBIT} gates.  %% DA: note that in safety people probably don't expect big trees on prevention input, just one label?

% semantics we present still preserve these semantics and allow to not deviate from the underlying DT formalisation, whilst more closely following the diagrammatic representations if the figures.
%The function \texttt{INHIBIT} is a binary function $\mathbb{B} \times \mathbb{B} \rightarrow \mathbb{B}$.


% \begin{definition}[Disruption Defence Tree]
% A disruption defence tree is a tuple $T = (N,t,\mathit{ch}, \delta)$ where:
% \begin{itemize}
%   \item $(N,t,\mathit{ch})$ is a disruption tree;
% %    \item $N$ is a finite set of nodes
% %    \item $t: N \rightarrow \mathbb{T}$ gives the type of each node
% %    \item $ch: N \rightarrow N^*$ gives the sequence of children of a node
%     % \item $L$ id labels setting attacker and defender roles
%     \item $\delta : N \rightarrow \mathbb{L}$ is a %% n injective   DA: I don't think so, that would mean only two nodes!
%     function assigning labels to the nodes
%     %\item $act: N \rightarrow \{a,d\} $ 
%     %is a function assigning actors to the nodes 
%     in such a way that 
%     $\forall n\in N. \exists u \in ch(n).\delta(u) \neq \delta(n)$
%     %every node has at most one node assigned to the child of an actor of the opposite kind. 
% \end{itemize}
% Moreover, T satisfies the following constraints:
% \begin{itemize}
%   \item the label assigned to the root node signifies whether the goal is to disrupt or correct the system.
% %   \item \texttt{LEAF} nodes by definition will have no children according to this formalisation as any node with children is a gate (this will be discussed further in the section on operations for interdependence Sec.~\ref{sec:operations}).
% \end{itemize}
% \end{definition}

\subsubsection{Structure of a DPT}

The semantics of a DPT allows a proponent to block an opponent.  These kind of barriers are called ``avoid barriers'' in fault trees~\cite{de2006aramis,guldenmund2006development} and ``defences'' in attack trees~\cite{kordy2010foundations}, but function in the same manner.
% Note that the graphical notation uses \texttt{INHIBIT} gates to represent barriers,
Following from the DT semantics~\cite{stoelinga2021marriage}, we generalise the structure function to interpret the
additional gate.
% of a disruption tree $T$ is a function $f_T : \mathbb{B}^n \rightarrow \mathbb{B}$.
% T vector $v = \langle v_1, . . . ,v_n \rangle$ indicates for each leaf $i$ whether it
% was disrupted, i.e., $vi = 1$ if leaf $i$ has failed or was attacked. 
% Then $f_T(v) \in \{0, 1\}$ indicates whether the whole system was disrupted. 
% This function can be defined recursively in the nodes of $DPT:f_T (v, A)$ tells whether $A \subseteq \text{\texttt{LEAF}}$ suffices to disrupt node $v \in N$ of $T$, where $A$ encodes $v$ as usual.



\begin{definition}[Structure function for DPTs] %
  \label{def:DPT-sems}
  The structure function $f_T:N\times2^{\leavesof{T}}\rightarrow\mathbb{B}$ of a DPT $T$ and
  $A \subseteq \text{\texttt{LEAF}}$ is defined by:\\
  \begin{displaymath}
    f_T(v,A) = %
    \begin{cases}
      \TRUE &  \begin{cases}%
                        \mathrm{if}\ t(v)=\ORt & \mathrm{and}\ 
                                    \exists u \in \ch(v).\ f_T(u,A) = \TRUE
                        \\%
                        \mathrm{if}\ t(v)=\ANDt & \mathrm{and}\ 
                      \forall u \in \ch(v). \ f_T(u,A) = \TRUE
                        \\%
                        \mathrm{if}\ t(v)=\INHIBITt & \mathrm{and}\ 
                        f_T(u_1,A) = \TRUE, f_T(u_2,A) = \FALSE
                        \ \mathrm{where}\ \ch(v)=[u_1,u_2] \\
                        \mathrm{if}\ t(v)=\LEAFt & \mathrm{and}\ 
                        v\in A 
               \end{cases}  \\%
      \FALSE & otherwise%
    \end{cases}
  \end{displaymath}
  The interpretation for the overall tree is $f_T(A) = f_T(R_T,A)$.
\end{definition}  
\noindent
% said above now
% The semantics of a DPT generalises those of a DT %see Stoelinga et al.~
% \cite{stoelinga2021marriage,budde2021attack}, allowing nodes to inhibit inputs, to capture barriers. 
%% DA: what about comparison to attack-defence trees? [above now]
%% DA: this remark refers to previous definition
%% Prevention assessments assume proponents and opponents operating one after another in turn (inferred from the negated inputs); note that the barrier action (when the polarity changes) is treated conjunctively for both \texttt{OR} and \texttt{AND} nodes. 

% \textcolor{red}{Proponent function}

%% DA: this is what we want right?

%% DA: some remark also about NOT gates
%% may be in order, presumably could
%% express this already if we're boolean
%% complete.  We should explain why
%% tree structure isn't boolean complete or more general,
%% something to do with 

% $ch(v)$ of a different label type will instead be considered an inhibited input to the gate $t(v)$. 

%% DA: I think (a nested) example might help at some point

We will sometimes use syntactic notation to construct DPTs using \texttt{AND} (written as $\cap$), \texttt{OR} ($\cup$) and \texttt{INHIBIT} ($\hexagon$) as term constructors and label
names to stand for nodes in the graph.  This can be made formal by defining interpretation functions on terms (for example,
see~\cite{jhawar2015attack}).




\subsection{Consequence Assessments}
\label{sec:right}

A consequence assessment constitutes the right hand side of a safety-security bowtie and investigates potential ways to mitigate the central risk event or negative outcomes.
As usually done with bowties, we make use of event trees to investigate each possible outcome of the central risk event.
For the RHS of the bowtie, the leaf nodes in the DCT are potential
final consequence events and each \CHOOSEt node represents a splitting
point where a sub-event can have different outcomes (typically for a
binary choice point, something happens or does not happen).  This is
captured by a \emph{consequence function} $C$ which selects the
outcome event at each \CHOOSEt node, tracing a path through to a final
outcome.  For the Boolean interpretation only a single choice can
happen; for more general interpretations we might assign a possibility
(Y/N/M) against each branch, probabilities or probability
distributions, etc.
% To construct the tree each event ($n$) is considered sequentially and constitutes a branching of a tree, one branching on $n$ takes place (as $develop(n)$) and one does not taken place (as $suppress(n)$).
% % We so for each node $n$ we can label these as $develop()$ and $repress()$
% % Each branching of this kind has a probability likelihood summing to one,
% Eventually each branch will lead to a final outcome of the system~\cite{pate1984fault}, as a terminal $\text{\texttt{LEAF}}$ node of type $\mathbb{B}=\{1,0\}$.

% We note that each event in the tree will be conditional on its antecedent event.
% An event in the tree is of 
% \textcolor{red}{We further add two types of barriers, prevent control barriers and limit barriers following in line with previous literature~\cite{de2006aramis}}.
% \begin{definition}[Disruption Recovery Tree]
% A Disruption Recovery Tree (DCT) can be viewed as a tuple $D = (E,t,ch)$ where:
% \begin{itemize}
%     \item $E$ is a finite and ordered set of event nodes $(e_1,...,e_n)$ where $e_1 < ... < e_n$
%     \item $t:E \rightarrow \mathbb{E}$ gives the type of each event node where $\mathbb{E}=\{\text{\texttt{LEAF}}, \text{\texttt{SWITCH}}\}$
%     \item $ch:E \rightarrow E^*$ gives the sequence of children of a note
% \end{itemize}
% %LA: need these??
% % Like previous definitions $D$ is a rooted DAG and as such:
% % Moreover, T satisfies the following constraints:
% % \begin{itemize}
% %     \item $(N,E)$ is a connected DAG where $E = \{(v,u) \in N^2| u\in ch(v)\}$;
% %     \item $T$ has a unique root, denoted by $R_T:\exists ! R_T \in N . \forall v \in N. R_T \not\in ch(v)$.
% % \end{itemize}
% Similarly to previous definitions (where $\exists !$ stands for unique existence),%% DA: this is notational, not a constraint  
% we define $\leavesof{D} = \{ v\in E \;|\; ch(v)=\epsilon\}$ for the leaves of $D$.
% \end{definition}



% \begin{definition}[Structure function for DCT] \label{def:DCT-sems}
%     The structure function $f_D:E\times2^{\leavesof{D}}\rightarrow\mathbb{B}$ of a DCT $D$ is given by:\\
%     $f_D(u,A) =
%     \begin{cases}
%           \text{\texttt{\textbf{1}}}\ \ if \ t(v)=\text{\texttt{SWITCH}}\ \ \ \qquad and\ 
%           \exists 
%     \end{cases}$
% \end{definition}


\begin{definition}[Disruption Consequence Tree]
  \label{def:dct2}
  A Disruption Consequence Tree (DCT) is a structure tree with gate types $\mathbb{T} = \theset{\LEAFt, \CHOOSEt}$.
\end{definition}
% % LA: I tried. 
% \begin{definition}[Disruption Consequence Tree]
% % A Disruption Consequence Tree $DCT$ is a tree $\langle  N, t , ch \rangle$ as given by Def~\ref{def:dt}  with gate types $\mathbb{T} = \{\text{\texttt{LEAF}}, \text{\texttt{CHOOSE}}\}$.
% %   A Disruption Prevention Tree (DPT) is a DT in the form $T = (N,t,\mathit{ch})$ with gate types
% %   $\mathbb{T} = \{\text{\texttt{LEAF}},\text{\texttt{OR}},\text{\texttt{AND}}, \text{\texttt{INHIBIT}}\}$,
% %   with the constraint that \texttt{INHIBIT} nodes have exactly two children; the second child corresponds
% %   to the inhibiting (prevention) condition.
% A Disruption Consequence Tree $DCT$ is a tree $\langle  C, t, val, ch \rangle$ where:
% \begin{itemize}
%     \item $C$ is a ordered set of consequence, $[x_0,...,x_i] $ where $x_0 < ... < x_i$.
%     \item $t:C \rightarrow \mathbb{T}$ gives the type of each node where $\mathbb{T} = \{\text{\texttt{LEAF}},\text{\texttt{SWITCH}}\}$
%      \item $val(c) \rightarrow \mathbb{B}$ returns the value of the consequence
%     \item $ch:C \rightarrow C^*$ gives the sequence of children of a node.
%     % \item given an event $x$ the next state $s+1 \in S$ of the tree is calculated as a branching $x$ and $\Bar{x}$ at every vertex currently in the tree.
% \end{itemize}
% Moreover DCTs are subject to the following restrictions:
% \begin{itemize}
%     \item each event $e$ of type $\text{\texttt{SWITCH}}$ has exactly two outgoing edges denoted by $develop(e)$  and $repress(e)$. 
%     \item all events are unique such that $val(e_i) = val(e_j), develop(e_i) = develop(e_j),repress(e_i) = repress(e_j) \implies e_i = e_j,$
% \end{itemize}
% \label{def:DCT}
% \end{definition}




    \begin{definition}[Structure function for DCTs] %
      \label{def:DPC2-sems}
      The structure function $f_T:N\times({\choicesof{T}\to\mathbb{N}})\rightarrow N$ of a DCT $T$ is
      defined by:
      \begin{displaymath}
        f_T(v,C) = 
        \begin{cases}
          v & t(v)=\LEAFt \\
          f_T(u_n,C) & \mathrm{where}\ C(v)=n\ \mathrm{and}\ \ch(v)=[u_1,\ldots,u_n]
        \end{cases}                 
      \end{displaymath}
      where $C$ is a consequence function which selects
      an outcome for each \CHOOSEt node, i.e.,
      $1\leq C(v)\leq \mathit{length}(\ch(v))$ for $v\in\choicesof{T}$.
      The interpretation for the overall tree is $f_T(C) = f_T(R_T,C)$.
    \end{definition}

% \begin{definition}[Structure function for DCT] \label{def:DCT-sems}
% % A consequence is a node from the DCT together with a choice of outcomes $(v,i)$, where $t(v)= \text{\texttt{CHOOSE}}$ and $1 \leq i \leq len(ch(v))$. 
% % The final outcome of a DCT is the \texttt{LEAF} reached by a sequence of consequences, this is captured by a function $f_T$ which for each \texttt{CHOOSE} node will $ev:N \rightarrow \mathbb{N}$ an event $(v,ev(v))$ as:
% % $f_T(v,ev) = 
% %     \begin{cases}
% %           v \qquad \qquad \quad \quad if\  t(v) = \text{\texttt{LEAF}}\\
% %           f_T(ev(v),ev)\ \ \  if\ t(v) = \text{\texttt{CHOOSE}}
% %     \end{cases}$\\
% %     \smallskip
% %     And for the tree, $f_T(ev) = f_T(R_T,ev)$
%      The structure function $f_D:E\times2^{\leavesof{D}}\rightarrow\mathbb{B}$ of a DCT $D$:\\
%      $f_D(v,C) =
%      \begin{cases}
%           If \  t(v) = \text{\texttt{LEAF}}\quad \ \  then \ \quad
%           \begin{cases}
%               \text{\texttt{\textbf{1}}}\ \ if \ val(v) = 1 \quad and\ \ \forall u \in ch(v). F_D(u, C) =1 \\
%               \text{\texttt{\textbf{0}}}\ \ if \ val(v) = 0 \quad and\ \  \forall u \in ch(v). F_D(u, C) =0 \\
%           \end{cases}\\
%           If \  t(v) = \text{\texttt{SWITCH}}\ \  then \ \qquad
%                 \overline{v}\ \cdot\ f_D(suppress(v),C)\ \oplus\ v \cdot f_D(develop(v),C)
%      \end{cases}$\\
%      \smallskip
% %     And for the tree, $f_T(ev) = f_T(R_T,ev)$
% % The interpretation for the overall tree is $f_T(D) = f_T(R_T,C)$ 
% \end{definition}

% \begin{definition}[Structure function for DCT] \label{def:DCT-sems}
%      The structure function $f_D:E\times2^{\leavesof{D}}\rightarrow\mathbb{B}$ of a DCT $D$, and a  is given by:\\
%      $f_D(v,ev) =
%      \begin{cases}
%           If \  t(v) = \text{\texttt{LEAF}}\quad \ \  then \ \quad
%           \begin{cases}
%               \text{\texttt{\textbf{1}}}\ \ if \ val(v) = 1 \quad and\ \ \forall u \in ch(v). F_D(u, E) =1 \\
%               \text{\texttt{\textbf{0}}}\ \ if \ val(v) = 0 \quad and\ \  \forall u \in ch(v). F_D(u, E) =0 \\
%           \end{cases}\\
%           If \  t(v) = \text{\texttt{SWITCH}}\ \  then \ \qquad
%                 \overline{v}\ \cdot\ f_D(suppress(e),E)\ \oplus\ v \cdot f_D(develop(e),E)
%      \end{cases}$
% \end{definition}
% \smallskip

% Each of the possible outcomes of the tree, dictated by the \texttt{LEAF} of each branch is a function of all events on the branch.
% Calculated as the sequence $(c_0 \oplus \overline{c_0}|,...,|c_{f-1} \oplus \overline{c_{f-1}})$ where each $c_i$ corresponds to an event in the branch.



% \begin{definition}
    
%     The structure function $f_T:N\times2^{LEAF}\rightarrow\mathbb{B}$ of a disruption defense tree $T$ is given by:\\
%     $f_T(v,A) =
%     \begin{cases}
%           \text{\texttt{\textbf{1}}}\ \ if \ t(v)=\text{\texttt{OR}}\ and\ \exists\ \{u \in ch(v)\ | \  \delta(u) = \delta(v)\}\ .\ f_T(u,A) = 1 \\ 
%           \ \ \ \land \  \forall\ \{i \in ch(v)\ |\ \delta(i) \neq \delta(v)\}\ .\ f_T(i,A) = \neg f_T(u,A)\\    
%           \text{\texttt{\textbf{1}}}\ \ if \ t(v)=\text{\texttt{AND}}\ and\ \forall\ \{u \in ch(v) \ | \delta(u) = \delta(v) \}\ . \ f_T(u,A) = 1\\
%           \ \ \ \land \  \forall\ \{i \in ch(v)\ |\ \delta(i) \neq \delta(v)\}\ .\ f_T(i,A) = \neg f_T(u,A)\\    
%           \text{\texttt{\textbf{1}}}\ \ if \ t(v)=\text{\texttt{LEAF}}\ and\ v \in A,\\    
%           \text{\texttt{\textbf{0}}}\ \ otherwise\\    
%     \end{cases}$
% \end{definition}

% We note of the downsides of this approach is that the final states of the systems need to be manually analysed an labelled, as the branching contains no extra information about the final state of the system. 
% This means every outcome is composed simply of the series of events that led to it.

% \subsection{Formalisation of Dependencies}


% \subsection{Operations for Dependencies}

% \subsection{Probability of Outcomes}

% 
\subsection{Bowties}

% Given a DPT and a DCT we can join them by a top event, matching the \textit{root} of the DPT and the \textit{initial event} of the DCT, to form a completed bowtie.
A bowtie is just a pair of two structured trees.  Intuitively, the top event corresponds
to the two roots linked together, a realised disruption.  %% DRAW PICTURE
\begin{definition}[Disruption Bowtie]
  A Disruption Bowtie (DB) is a pair $\langle T_P, T_c \rangle$ of a disruption prevention
  tree and a disruption consequence tree.
\end{definition}


% \begin{definition}[Disruption Bowtie]
%   A Disruption Bowtie (DB) is a tuple $DB = (\mathcal{P},\text{\texttt{te}},\mathcal{C})$, whereby $\mathcal{P}$ is a well formed DPT as per  Def.~\ref{def:dpt}, $\mathcal{C}$ is a well formed DCT as per  Def.~\ref{def:DCT}, and $\text{\texttt{te}}$ is the top event of investigation where, $\mathcal{P} \rightarrow \text{\texttt{te}}$ corresponds to the outcome of $\mathcal{P}$, and $\text{\texttt{te}} \rightarrow \mathcal{C}$ is the initial consequence $c_0$ of $C$
% % \begin{itemize}
% \end{definition}



==> texts/interdependence.tex <==

\section{Interdependence Analysis}
\label{sec:dependencies}

When assessing the interactions between security and safety we categorize them following the existing literature~\cite{kriaa2015survey,eames1999integration}, they are:
\begin{enumerate}
    \item \textit{conditional dependency}, meaning the safety of the system depends on its security, and conversely, 
    \item \textit{mutual reinforcement}, fulfilment of safety requirements or safety measures contributes to security, and conversely, 
    \item \textit{antagonistic}, when considered jointly, safety and security requirements or measures lead to conflicting situations, and 
    \item \textit{independence}, when the interactions are mutually exclusive or not in interference.  
\end{enumerate}

% We will highlight examples of each of these in the scenarios and investigate how they can be modelled.
% Note that no previous attempt has formalised these dependencies in a structured manner.
The interactions, obviously, have a great difference on the result of the assessment and in our case study we see dramatic differences in the same exact events inter-playing in different ways.
% We note that certain gates, although uncommon in the base definition of disruption trees are essential when observing inter-dependencies, e.g. the XOR gate for antagonistic interactions.
We showcase in the scenarios the need for specific operations and describe their semantics in this section. 
We omit the right hand side of the bowtie for those interdependencies which do not strictly require it (\textit{independence} and \textit{conditional}).
Whilst we find that both \textit{reinforcing} and \textit{antagonistic} require the recovery side of the bowtie.
We note that each interdependency condition leads to trees joined in the usual fashion when combining to form a new tree.
% A full scenario analysis with recovery measures is omitted as it is orthogonal to this initial analysis of inter-dependency operators, however a future full paper dedicated to the interdependence of recovery measures would also potentially be beneficial.
% Now lets assume that these two events were happpening at the same time and explore their dependencies. 

%% ADD section 2.5 here. \subsection{formalise the example}
%% explain RSA is the same attack strategy but different event, RSA_1 and RSA_2, same attack but have independent occurance, in a DAG strusture they could be treated as same event if we wanted. 
%% introduce that these are joined as trees in the usual fashion when combining new tree.

\subsection{Running Example: Safety Security Interplay}
\label{sec:example}

% For the sake of case study we choose to adapt the attack tree from~\cite{jhawar2015attack}, and the safety incident with Facebook as the fault tree.
As main point of reference we use the reported chain of events by Facebook engineering~\cite{janardhan2021first,janardhan2021second} as well as the external assessment conducted by CloudFlare~\cite{martinho2021}.
We conducted a structured risk assessment of the Facebook DNS shutdown using security safety bowties focusing our analysis on how safety and security measures interacted to lead to the specific events.
Our methodology of analysis was the following: i) we downloaded the analysis of the events released by the Facebook engineering team as well as an external examination by cloud hosting provider CloudFlare which witnessed the events externally. ii) we systematically labelled each brief to extract events, its causes and outcomes and the recovery/preventions that were in place (and failed in this case).
For the sake of case study we choose to adapt an attack tree that reached the same risk event of the server outage, for this we borrow an existing example from~\cite{jhawar2015attack}.
For the sake of diagrammatic explainability edges are labelled by an identity function, which creates the intermediate events, a full table containing all edge labels is presented in Tab.~\ref{tab:edge-labels}.

\begin{table}[htb]
\caption{Explanations of edge and event labels.}
\label{tab:edge-labels}
\centering
\footnotesize
\begin{tabular}{p{0.145\linewidth}|p{0.35\linewidth} ||p{0.14\linewidth}|p{0.35\linewidth}}
\textbf{Attack Label }    & \textbf{Explanation}& \textbf{Safety Label}  & \textbf{Explanation} \\


\hline\hline
\textbf{Server Down}    & Once the attacker has gained access to the server he chooses to deny others access.  & \textbf{Server Down}   & Due to erros with DNS configuration and a faulty update with a failed check the server goes offline\\\hline

\textbf{auth}& Breaching the authentication mechanism & \textbf{faulty update} & Due to unchecked issues in patch the faulty update when't through\\\hline

\textbf{no auth} & Bypassing the authentication mechanism & \textbf{DNS OFF}       & Due to safety procedure DNS hidden from internet \\\hline

\textbf{user privileges} & Gain illegitimate privileges & \textbf{update check}    &  The safety checker for updates failed to spot the fault \\\hline

\textbf{buffer overflow}  & Exploit vulnerabilities to overflow & \textbf{dns check} & Internal safety procedure was that if the internal DNS resolver couldn't find its own address it removed the DNS from the internet \\\hline

\textbf{rsa} & RSAREF2 library buffer overflow vulnerability & \textbf{server patch}  & An engineer send an update to the backbone routers which was faulty \\\hline

\textbf{ssh} & ssh deamon overflow vulnerability & \textbf{resolve dns }  & DNS is unable to resolve its own addresss \\\hline

\textbf{rsh} & Remotely executing shell commands & \textbf{remote login} & Remotely patch the server to remove failure\\\hline
\textbf{ftp} & Exploit ftp vulnerability to upload files&&\\\hline
\textbf{server disrupt}   & Once the attacker has gained access to the server he alters the DNS settings &               & \\\hline
\textbf{disable ssh} & Remove ssh access to stop vulnerability &&\\
\hline             \hline                                                                                                             
\end{tabular}

%\label{tab:edge-labels}
\end{table}
% For the analysis in this work we further extrapolate that this server may have been a server hosted on the Facebook routing network during the DNS incident.
The triggering of the initial Facebook blackout was caused by two independent events, firstly an engineer sent an update to the backbone routers which was faulty, this was not caught by the safety checker and was allowed to go through.
An internal safety procedure was: that if the internal DNS resolver couldn't find its own address it removed the DNS from the internet, meaning they were invisible to the outside world.
% The fault tree in Fig.~\ref{fig:independence} shows how the faults led to the eventual server being down, labelled by the \texttt{safety cause} on the final edge.
In the case of an attack we consider a generic server, offering ftp, ssh, and rsh services, as seen in previous work~\cite{jhawar2015attack}. 
The attack tree in Fig.~\ref{fig:antagonistic} shows how an attacker can disrupt a server in two ways: either without providing any user credentials (no-auth) or by breaching the authentication mechanism (auth).
In the first case, the attacker must first gain user privileges and then perform a local buffer overflow attack.
To gain user privileges, the attacker must exploit an FTP vulnerability to anonymously upload a list of trusted hosts as well as remotely executing shell commands using RSH. 
The second way is to abuse a buffer overflow in both the ssh daemon (SSH) and the RSAREF2 library (RSA) used for authentication.




Using the described notation we formalise the security and safety scenarios as $DPT_S$ and $DPT_A$ for safety and security respectively:
\begin{equation*}
    DPT_S = ((\text{\texttt{server patch}}\ \hexagon\ \text{\texttt{update check}})\cap(\text{\texttt{resolve DNS}}\ \hexagon\ \text{\texttt{dns check}})) 
\end{equation*}
\begin{equation*}
    DPT_A =  ((\text{\texttt{ftp}}\ \cap\ \text{\texttt{rsh}})\ \cap\ \text{\texttt{buffer overflow}})\ \cup\ (\text{\texttt{rsa}}\ \cap\ \text{\texttt{ssh}})
\end{equation*}


% \begin{itemize}
%     \item INSERT tree booleans here.
% \end{itemize}



% \begin{figure} [htbp!]
%     \centering
%     \includegraphics[width=\textwidth]{figs/Safety_Tree.png}
%     \caption{Fault Tree Scenario}
%     \label{fig:attack-scenario}
% \end{figure}

% \subsection{Combined Scenario}

% \begin{itemize}
%     \item exaplain each of the interdependencies
% \end{itemize}


\subsection{Independence}

%  is probably the easiest type of dependence to model, both for construction and analysis.
The Independence relationship can simply be defined as an \texttt{OR} gate, whereby either the security scenario \textit{or} the safety scenario lead to the eventual risk condition, an initial investigation of this has has been done before~\cite{steiner2013combination}, and can be visualised in Fig.~\ref{fig:independence} for our case study.



For quantitative analysis there are, however, certain complications.
Since now both a safety assessment is present as well as a security assessment, there needs to be a choice as to how the OR gate quantification is performed.
Whilst this topic in itself warrants a deeper discussion orthogonal to the contributions of this work, a naive approach is to employ the approach from Steiner and Liggesmeyer and calculate a composition of risk-probability pairs leading to the \texttt{OR} gate outcome~\cite{steiner2013combination}.
In the case study we simple see that the server outage may be caused by an active attacker (attack tree), or a failure of the update process and DNS misconfiguration (safety tree), or both.

%% elipsis on right hand side 
%% elipsis into security and safety case. 
%% add to caption to say it's a fragment to figure one.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/case-study-independence-short.pdf}
    \caption{Independence - when the two events do not interact to cause the final outcome. This is a sub-tree of the tree in Fig~\ref{fig:antagonistic}, and as such details are omitted}
    \label{fig:independence}
\end{figure}

%%%% ADDED
Independence is modelled as two DPTs joining roots with an \texttt{OR} gate.
\begin{definition}
An independent joining of  a security and a safety assessment (assuming both are modelled as disruption defence trees) is defined as: given two disruption defence trees $DPT_{A}$ and $DPT_{F}$ a new tree $DPT_{AF}$ is formed as:
\begin{itemize}
    % \item $DPT_{AF}$ has a unique root, denoted by $RT_{ind}:\neg\exists\  RT_{ind}\  \in N_{AF}\ .\ \forall v \in N_{AF} . RT_{ind} \not\in ch(v)$
    % \item  $RT_{ind}\  \in N_{AF} \ . \ t:RT_{ind} \rightarrow \text{\texttt{OR}}$
    % \item Given the previous vertices of $DPT_{att}$ and $DT_{fault}$, $RT_{att}$ and $RT_{saf}$, the children of  will be $ch:RT_{ind} \rightarrow (RT_{att},RT_{saf})$
%    \item $DPT_{AF} := (N_A \uplus N_E \uplus \{R_{T_{AF}}\}),\ t_a \uplus t_f \uplus \{\{R_{T_{AF}}\rightarrow \text{\texttt{OR}}\},\  ch:R_{T_{AF}} \rightarrow (R_{T_{A}},R_{T_{F}})$
    \item $DPT_{AF} := \langle\, 
        N_A \uplus N_E \uplus \{R_{T_{AF}}\},\ 
        \mathbb{T}, \
        t_a \uplus t_f \uplus \{R_{T_{AF}}\mapsto \text{\texttt{OR}}\},\  
        ch_{A} \uplus ch_{F} \uplus \{R_{T_{AF}} \mapsto [R_{T_{A}}, R_{T_{F}]} \} \rangle$
     %% OR:
     %% DPT_{AF} = DPT_A\; \texttt{OR}\; DPT_F
     %% 
 \end{itemize}
\label{def:ind}
\end{definition}

So for the example in Fig.~\ref{fig:independence}, the independent joining would look like this:
\begin{equation*}
\begin{split}
     FB_{IND} = &  ( ((\text{\texttt{ftp}}\ \cap\ \text{\texttt{rsa}})\ \cap\ \text{\texttt{buffer overflow}})\ \cup\ (\text{\texttt{rsa}}\ \cap\ \text{\texttt{ssh}}))\ \ \cup \\
 & ((\text{\texttt{server patch}}\ \hexagon\ \text{\texttt{update check}})\cap(\text{\texttt{resolve DNS}}\ \hexagon\ \text{\texttt{dns check}}))
\end{split}
\end{equation*}




\subsection{Conditional Dependency}


% Conditional dependency requires further operations for construction. 
Given two disruption prevention trees a conditional dependence means that the vertex of one of the trees corresponds to a child node or intermediate event of the other.
A conditional joining extends the tree to include all the children of the vertex being merged in, with the old vertex simply becoming an intermediate event to the other tree.
The assessment now needs to include all the new nodes that lead to the risk event.
In the example we can easily presume that the failure to resolve the DNS could be due to an attacker having gained access to the server (following the attack path from the attack tree) and changing the configuration.
So by merging the attack tree to the fault tree on the resolve DNS node we get a conditional dependence, as seen in Fig.~\ref{fig:conditional}.

%%  can be 0.7
\begin{figure} [htbp!]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/case-study-conditional-leaf.pdf}
    \caption{Conditional - when the safety outcome is conditional on the security  or vice versa. Scenario modelled by security  outcomes (simplified) causing fault.}
    \label{fig:conditional}
\end{figure}

%%% ADDED
A conditional dependence may be viewed as the expansion of a previously unknown external event.
Whilst previously we had a \texttt{LEAF} node that represented an input to an assessment, we now expand this node into a fully fledged disruption tree.
This notion of external event is seen in previous literature~\cite{vesely1981fault}, and this can be seen as an enhancement of knowledge of what lead to the input events.
Semantically it means that a node at the bottom of a disruption tree simply gains as children all the nodes in another disruption tree, and the previous child leaf node is substituted.

%% FIX to include all tuples for this and DEF 6
\begin{definition}
A conditional joining of  a security and a safety assessment (assuming both are modelled as a disruption defence tree) is defined as: given a joining of two disruption defence trees $DPT_{A}$ to $DPT_{F}$ and a condition node $n_c$ (of type \INHIBITt) a new tree $DPT_{AF}$ is formed as:
\begin{itemize}
    % \item $DPT_{AF}$ has a unique root, denoted by $RT_{fault}$
    % \item for a given final node in $n \in RT_{fault}$ where $\forall\ i\ \in ch:n \rightarrow (\text{\texttt{LEAF}})$ the joining will result in $ch:n' \rightarrow ch:n \cup N_{sec}$
    % UPDATE: ch:n_c is a LEAF so we do not map children to it, we map nc to the new tree
    \item  $DPT_{AF} := \langle N_A \uplus N_F \uplus \{n_c \mapsto R_{T_A}\}, \mathbb{T}, t_A \uplus t_F \uplus \{t_{AF}(n_c) := t_A(R_{T_A})\}, ch_{A} \uplus ch_{F} \rangle$
   
\end{itemize}
\end{definition}

So for the example in Fig.~\ref{fig:conditional}, the conditional joining would look like this:
\begin{equation*}
\begin{split}
     FB_{COND} = & ((\text{\texttt{server patch}}\ \hexagon\ \text{\texttt{update check}})\ \cap \
      ((\text{\texttt{rsa}}\ \cap\ \text{\texttt{ssh}})\ \hexagon\ \text{\texttt{dns check}}))
\end{split}
\end{equation*}



\subsection{Reinforcing Dependency}
\label{sec:reinforce}
% \begin{itemize}
%     \item need NOT gate to show security response fixing safety incident
%     \item need outcomes
% \end{itemize}

The reinforcement dependency takes place when a DCT from one bowtie contains a response/outcome that leads to the resolution of the initial scenario of a separate DPT.
This means that due to the response to an incident another incident is no longer plausible.
If we take the same security response as previously, disabling ssh to stop the buffer overflow, we see that the patching of the server event which led to the faulty update cannot take place anymore, as per Fig.~\ref{fig:reinforce}.
This once again requires the right hand side of a bowtie.
In this scenario the response outcome of one bowtie is chaining to the cause event of another tree.
Concretely, the response \texttt{disable ssh} negates the \texttt{server patch} event of the fault tree.
This is modelled through a \texttt{INHIBIT} gate.
Simply this is evaluated as the action no longer being possible (as the response is not negated it results to 0 in \texttt{INHIBIT} semantics).

%%  can be 0.6 or 07
\begin{figure} [htbp!]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/case-study-reinforcement-leaf.pdf}
    \caption{Reinforcing - when a security or safety measure helps the other incident. This is modelled by the outcome of security (simplified) in this case, stopping the safety incident. Attack tree omitted as it is sub-tree of Fig.~\ref{fig:antagonistic}}
    \label{fig:reinforce}
\end{figure}


Reinforcing dependence assumes that as an outcome of fixing a fault or mitigating an attack, another fault or attack is no longer possible.
% This, in practice, negates a disruption in the disruption defence tree which is being reinforced, which may in some cases make it so that a risk event is no longer possible, as per our case study (see Sec.~\ref{sec:reinforce}).
% For the sake of maintaining the semantics, which allows for much more flexibility and modularity, there is no joining of the tree's but rather an analysis that leads to the alteration of the reinforced tree.
% More specifically if a recovery event is present in the event tree that fixes a fault or mitigates an attack event in the disruption tree, than that event is set as negated for the tree.
% As discussed previously, reinforcing dependencies require outcomes/responses to be expressed (right hand side of a bowtie).
The approach taken in this scenario is to take the DCT on the right hand side of the bowtie, joining into the reinforced DPT, extending it, and creating a new DPT.
This leads to the final risk event of the reinforced DPT being the new risk event of focus for the whole assessment.
 We make the assumption that if an event does not lead to any other disruptions in the DPT being reinforced it is not influencing the disruption and can be pruned.
 (to preserver the tree structure and avoid back propagating branches). 
We infer that if an event is present in both trees there is an implied relationship, extensions could instead assign further labels to construct these relationships.

% INHIBIT
\begin{definition}
A reinforcing joining of a disruption consequence assessment (implicitly joining any left most side $DPT$ if a bowtie) $DCT$ and any disruption defence tree $DPT$ takes the form of a joining of the single reinforcing branch $V_C = f_T(R_T \in DCT,C)$ into a node $n_r$ of type \INHIBITt:
\begin{itemize}
    %\item for $N \in DPT$ and $E \in  DCT$ if $\exists(i . ch:N \rightarrow \{\text{\texttt{LEAF}}\})\in E)$ then $i' = \neg i$
    % so, the second child of n_r becomes V_n
    % 
    \item  $DPT_{AF} :=  \langle N \uplus V_C  
    %\uplus \{\text{\texttt{INHIBIT}}\} DO NOT NEED NEW NODE it is already INHIBIT
    , \mathbb{T}
    ,t_P \uplus t_C, % types do not change 
    ch_P \uplus ch_C \uplus % children stay same except, u1,u2 of nc
    \{ch_{PC}:n_r \mapsto [u1,\overline{V_C}]\}
    $
    %\{ch_{PC}:n_r\ \hexagon\ \overline{V_C}\}\} \rangle $ OLD
    
    % \item $DPT_{AF} := (N_A \uplus N_E \uplus \{R_{AF}\}),\ t_a \uplus t_f \uplus \{\{R_{AF}\rightarrow \text{\texttt{OR}}\},\  ch:R_{AF} \rightarrow (R_{A},R_{F})$
\end{itemize}
\end{definition}

%% CLEARED, now second child is replaced, which was prevention now is also precention gotten from other tree
We note that an inherent relationship between prevention and disruptions is assumed. 
This is not automatically inferred through formalisations.
In this case a prevention, child two of the \INHIBITt gate, is replaced by the branch of the DPT that reinforces the first child.
We see that the previous child two $u2$ of the \INHIBITt node is replaced by the branch $V_C$.
One can observe that under this formalism some knowledge about the previous events are lost, as they are pruned in the joining.
For clarity, an example joining between $DCT_i$ and $DPT_j$:
\begin{equation*}
    DPT_i = (\text{\texttt{X}}\ \hexagon\ \text{\texttt{Y}}) \ \text{and}\ DCT_j = ([j_i\cup \overline{j_i},j_n \cup \overline{j_n}])
\end{equation*}
if $j_n$ is reinforcing to \texttt{X}, their reinforcing joining $DPT_{ij}$, joins the path $V_j =\{j_i,j_n\}$ to $DPT_i$
\begin{equation*}
    DPT_{ij} = (\text{\texttt{X}}\ \hexagon\ \overline{V_j} )
\end{equation*}
%% EDITED
% We note this representation of a path of potentially several actions may be seen as a hierarchical label, whereby a path to an event is simply boxed to represent a single event.


\subsection{Antagonistic Dependency}

When security and/or safety measures directly antagonise each other it means that a measure that attempts to make the system more secure has an adverse effect on its safety and conversely.
% Colloquially, in an example of a nuclear power plant if there is a warning, the safety engineer will open all the doors, which would allow people to exit the building safely (but letting intruders in), conversely, a security engineer would close all the doors to keep the intruders out (but closing the people in). 
% This typical example showcases a clear scenario whereby a response completely rational for one sub-field is antagonistic to the other.
We see that this antagonism is almost exclusively present in an outcome of an incident taking place (i.e. after the warning has gone off), and not visible in the bare DPT.
For this specific scenario we need the use of the right hand side of a bowtie and event trees to represent the dependency.
Going back to our case study, once the server has been taken down, engineers from the safety domain and the security domain investigate the incident.
The first team (safety), sees that the incident is due to a faulty DNS configuration and patches the DNS remotely through SSH.
The second team (security), sees that the incident is due to a vulnerability in the ssh library and therefore disables ssh (perhaps temporarily whilst the issue is being fixed by local engineers, as was the case for Facebook).
As one can see, if the security response is put in place, there is no way the safety response can be put in place, this means that the fault or incident cannot be fixed if the security incident is fixed.
We note this is exactly what took place during the Facebook outage, a security response disallowed the safety engineers to remote in and patch the fault, leading to physical access being required.
% To represent this antagonistic relationship we make use of a \texttt{XOR} gate, only allowing one response but not both, as seen in Fig.~\ref{fig:antagonistic}.
In practice this means that the system can either be made safe or it can be made secure, but not both.
This unlike the previous relationships is modelled through the consequence assessment and through the usage of event trees.


\begin{definition}
An antagonistic joining of  a security and a safety consequence is defined as: given a joining of two disruption consequence assessments  $DCT_{A}$ and $DCT_{F}$, and antagonistic event $e$, a new tree $DCT_{AF}$ is formed as:
\begin{itemize}
    % \item $E_{AF} \in DCT_{AF}$ is given by a union between $E_{att} \in DCT_{att}$ and $E_{fault} \in DCT_{fault}$
    % \item given antagonistic event $a_e \in E_{AF}$ caused by $a_e = (e_{sec} \in E_{att}) \cup \Bar{ (e_{saf} \in E_{saf})}$ the next state $s+1 \in S_{AF}$ the branching will be calculated as $a_e$ and $\Bar{a_e}$
    % \item $a_e$ and $\Bar{a_e}$ determines that either $e_{sec}$ can take place but not $e_{saf}$ or conversely.
    \item $DCT_{AF} := \langle N_a \uplus N_s, \mathbb{T},  t_a \uplus t_s, ch_s \uplus ch_a \uplus \{ch_{sa}:e \mapsto \text{\texttt{CHOOSE}} \} \uplus  \{ch_{sa}:\overline{e} \mapsto \text{\texttt{CHOOSE}} \}  \rangle$, 
\end{itemize}
\label{def:antagonistic}
\end{definition}


finally the  Facebook DNS Disruption as a Bowtie can be defined in the following steps, given the $DPT_S$ and $DPT_A$ from Sec.~\ref{sec:example} they can be \textit{independently} joined following Def.~\ref{def:ind} to form:
\begin{equation*}
\begin{split}
 FB_{DPT} = &  ( ((\text{\texttt{ftp}}\ \cap\ \text{\texttt{rsh}})\ \cap\ \text{\texttt{buffer overflow}})\ \cup\ (\text{\texttt{rsa}}\ \cap\ \text{\texttt{ssh}}))\ \ \cup \\
 & ((\text{\texttt{server patch}}\ \hexagon\ \text{\texttt{update check}})\cap(\text{\texttt{resolve DNS}}\ \hexagon\ \text{\texttt{dns check}})) 
 \end{split}
\end{equation*}
\noindent and then given the two possible consequence trees, ${[DCT_A,DCT_S]}$:
\begin{equation*}
   DCT_S = (\text{\texttt{remote login}})\ \text{and}\ DCT_A=(\text{\texttt{disable ssh}})
\end{equation*}
\noindent we can antagonistically join them following Def.~\ref{def:antagonistic} to form the FB case study situation of conflict:
\begin{equation*}
\begin{split}
FB_{DCT} = & (\text{\texttt{remote login}}\ \cap\ \overline{\text{\texttt{disable ssh}}})\ \cup\ (\overline{\text{\texttt{remote login}}}\ \cap\ \text{\texttt{disable ssh}}) \\
& \text{ or more simply }(\text{\texttt{remote login}}\ \oplus\ \text{\texttt{disable ssh}}). 
 \end{split}
\end{equation*}
Putting the two together you can obtain the bowtie $FB_{Bowtie} = [FB_{DPT} \rightarrow [[\text{\texttt{server outage}} ]] \rightarrow FB_{DCT}]$


% \begin{itemize}
%     \item need for XOR gate
%     \item if security measure, outcome or barrier, safety no longer possible (note, this is safety of the system not safety incident)
% \end{itemize}
% Quantification of this is particularly nice as, its exclusivity removed the ambiguity of the \texttt{OR} gate calculations, the probability of an event is the probability of one input and the probability of the other input not taking place.

% \begin{itemize}
%     \item Do security Scenario
%     \item Do safety scenario
%     \item do the 4 types of merges
% \end{itemize}



%%%%% ALL THE CASES DO LATER

% Scenarios for each case:
% \begin{figure}[htbt!]
%     \centering
%      \begin{circuitikz} \draw
%         (1,2) node[or port, fill=none] (myor) {}
        
%         (myor.in 1) node[left =.2cm] (a) {A}
%         (myor.in 2) node[left =.2cm] (b) {B}
%         (myor.out)  node[right=.2cm] (c) {C}
        
%         (myor.in 1) -- (a)
%         (myor.in 2) -- (b)
%         (myor.out)  -- (c);
%         \end{circuitikz}
%     \caption{OR relationship}
%     \label{fig:my_label}
% \end{figure}
% \begin{center}
%     Scenario With OR Gate Security
% \end{center}
% \begin{center}
%     Scenario With OR Gate Safety
% \end{center}
% Scenarios for each case:
% \begin{figure}[htbt!]
%     \centering
%      \begin{circuitikz} \draw
%         (1,2) node[and port, fill=none] (myand) {}
        
%         (myand.in 1) node[left =.2cm] (a) {A}
%         (myand.in 2) node[left =.2cm] (b) {B}
%         (myand.out)  node[right=.2cm] (c) {C}
        
%         (myand.in 1) -- (a)
%         (myand.in 2) -- (b)
%         (myand.out)  -- (c);
%         \end{circuitikz}
%     \caption{AND relationship}
%     \label{fig:my_label}
% \end{figure}
% \begin{center}
%     Scenario With AND Gate Safety
% \end{center}
% \begin{center}
%     Scenario With AND Gate Security
% \end{center}

% \begin{table}[htbp!]
%     \centering
%         \caption{Symbols and Relationships in a fault tree}
%     \begin{tabular}{c|p{0.7\columnwidth}}
%     \hline
%     \multicolumn{2}{c}{\textbf{Event Types}}\\\hline
%      \noalign{\smallskip}
%       \tikz \draw (2,2) ellipse (10pt and 10pt); & \textit{Initial cause event} - initial fault requiring no further development \\
%       &\\
%      \fboxsep=6pt \fboxrule=0.5pt \fcolorbox{black}{white}{\phantom{\vrule width 8pt height 3pt}}    &   \textit{Intermediate cause event} - cause event as an outcome of relationship between previous events \\
%          &  \\ 
%     \centering \tikz \draw (0,0) ellipse (12pt and 8pt);   &   \textit{Prevention } - specific conditions that apply to a relationship i.e. this must fail in order to progress \\
%          &  \\ \hline
%   \multicolumn{2}{c}{\textbf{Relationship Types}}\\\hline
%          \noalign{\smallskip}
%     \resizebox{50pt}{20pt}{%
%   \begin{circuitikz} \draw
%         (1,2) node[or port, fill=none] (myor) {}
        
%         (myor.in 1) node[left =.2cm] (a) {A}
%         (myor.in 2) node[left =.2cm] (b) {B}
%         (myor.out)  node[right=.2cm] (c) {C}
        
%         (myor.in 1) -- (a)
%         (myor.in 2) -- (b)
%         (myor.out)  -- (c);
%         \end{circuitikz}}&   OR - output fault occurs if at least one of the input faults occurs\\
%         \resizebox{50pt}{20pt}{%
%   \begin{circuitikz} \draw
%         (1,2) node[and port, fill=none] (myor) {}
        
%         (myor.in 1) node[left =.2cm] (a) {A}
%         (myor.in 2) node[left =.2cm] (b) {B}
%         (myor.out)  node[right=.2cm] (c) {C}
        
%         (myor.in 1) -- (a)
%         (myor.in 2) -- (b)
%         (myor.out)  -- (c);
%         \end{circuitikz}}&   AND - output fault occurs if both of the input faults occurs\\
         
%         \resizebox{50pt}{20pt}{%
%   \begin{circuitikz} \draw
%         (1,2) node[xor port, fill=none] (myor) {}
        
%         (myor.in 1) node[left =.2cm] (a) {A}
%         (myor.in 2) node[left =.2cm] (b) {B}
%         (myor.out)  node[right=.2cm] (c) {C}
        
%         (myor.in 1) -- (a)
%         (myor.in 2) -- (b)
%         (myor.out)  -- (c);
%         \end{circuitikz}}&   XOR - output fault occurs if exactly one of the input faults occurs\\
%         \resizebox{30pt}{30pt}{%
%   \begin{tikzpicture}
%           \newdimen\R
%         \R=2.7cm
%           \draw (0:\R)
%           \foreach \x in {60,120,...,360} {  -- (\x:\R) }
%         -- cycle (360:\R) node[right] {}
%         -- cycle (300:\R) node[below] {}
%         -- cycle (240:\R) node[below] {)}
%         -- cycle (180:\R) node[left] {}
%         -- cycle  (120:\R) node[above] {}
%         -- cycle  (60:\R) node[above] {};
%         \end{tikzpicture}}
%                           &   INHIBIT - output fault occurs if the single input fault occurrs in the presence of an enabling conditions (represented by a prevention failing)\\\hline
%     \end{tabular}

%     \label{tab:symbols}
% \end{table}

% \subsection{The Case for Dynamic Prevention Assessments}
% \label{sec:left2}

% \begin{figure}[htbt!]
%     \centering
%       \begin{tikzpicture}
%           \newdimen\R
%         \R=1cm
%           \draw (0:\R)
%           \foreach \x in {60,120,...,360} {  -- (\x:\R) }
%         -- cycle (360:\R) node[right] {}
%         -- cycle (300:\R) node[below] {}
%         -- cycle (240:\R) node[below] {}
%         -- cycle (180:\R) node[left] {}
%         -- cycle  (120:\R) node[above] {}
%         -- cycle  (60:\R) node[above] {};
%         \end{tikzpicture}
%     \caption{INHIBIT relationship}
%     \label{fig:my_label}
% \end{figure}
% \begin{center}
%     Scenario With INHIBIT Gate Security
% \end{center}
% \begin{center}
%     Scenario With INHIBIT Gate Safety
% \end{center}

% \begin{figure}[htbt!]
%     \centering
%       \includegraphics[width=0.44\textwidth]{figs/andwithfeedback.png}
%     \caption{SAND relationship}
%     \label{fig:my_label}
% \end{figure}

% \begin{center}
%     Scenario With SAND Gate Security
% \end{center}
% \begin{center}
%     Scenario With SAND Gate Safety
% \end{center}










% \begin{itemize}
%     \item Introduce notation for even tree
%     \item Introduce notation for attack tree
%     \item do probabilities if time

% \end{itemize}

% \begin{itemize}
%     \item 
%     \item previous work has a risk assessment labelling function we assume it inherently (also deals with integrity)
%     \item we distinguish by the type of cause and outcome deliberately, hence fixing the structure of the left and the right.
%     \item previous work has a mapping function for type, description and proability, we see these as unnacessary and inherent in the node structure.
% \end{itemize}


% In its simplest form a SSB is defined as:
% \begin{theorem} Security Safety Bowtie. 

% % Let $e$ be a risk event who is the source of the current investigation, then $c \subset C$ is a cause of the event linked to $E$ by a connector ralation  Simple
% % is a continuous function.
% \label{the:simple}
% \end{theorem}

%\input{texts/formals/initial}
% \input{texts/formals/quantification}
%\input{texts/formals/prevention-recovery}
% \input{texts/formals/risk}
% \input{texts/formals/mergin}
% \input{texts/formals/chaining}




==> texts/introduction.tex <==

\section{Introduction}

% Thesis statement
%% DA: this seems like background/related work, let's get moving more quickly
% Although safety and security share many similarities and they both deal with risks, there are key differences when conducting these two types of assessments. 
% This in simple terms may refer to the distinction that system safety deals with ensuring the system does not impact the environment in a negative way; and conversely security of a system is aimed at preventing the environment from negatively impacting the system~\cite{line2006safety,pietre2010sema}. 
% Another difference between safety and security is the origin of risk: safety considers hazards, such as bad outcomes of system failures, whilst security considers threats and focuses on how potential attacks may impact the system's assets and its operation due to vulnerabilities.
% This generally in turn leads to the consideration of safety dealing with unintentional events, whilst security dealing with intentional malicious events.
%% Nonetheless despite these distinctions the interplay between these two fields is necessary as they are inherently deeply connected~\cite{bloomfield2013security}. 
% Safety techniques are very well studied and have been around for several years~\cite{line2006safety}, not only in the field of informatics but across a variety of field such as aeronautics~\cite{denney2015formal}, oil and gas industry~\cite{shahriar2012risk} and many more~\cite{inge2007safety}.
%% Security, although well studied, has been analysed in a less applied way and only recently have the same structured techniques, been applied in the same way to real world examples~\cite{bernsmed2017visualizing}.
%% However, with the advancement of technologies such as the internet of things giving unprecedented access to infrastructure for a malicious attacker, security will be required as a key part of any informed safety case; as if an attacker has access to the system, and the system is not secure the system will also not be safe~\cite{bloomfield2013security}.

% Standards for safety and security
% Several different standards exist for assessing risks to a system, and evaluating its safety and/or security. IEC 31010:2019 provides guidance on the selection and application of various techniques that can be used to help improve the way uncertainty is taken into account and to help understand risk. They specify these techniques are used to gain understanding about potential risks your system may face, comparing the risks of multiple decisions, mitigation of risks and assessment of mitigations. NIST.SP 800-30 dictates a process to conduct a risk assessment from scratch.  ISO/IEC 15408 provides guidance for obtaining for computer security certification. More generally speaking general assessment criterias are proposed for conducting safety assessments, such as  STAMP (System-Theoretic Accident Model and Processes)~\cite{leveson2016engineering} for identifyiying safety risks of a system or the Industrial Control Cyber Killchain~\cite{assante2015industrial}, for finding attacks on ICS settings. 
% These can all be unified in the application of structured reasoning to discover risk, threats and hazards to a system.
% However they still need to be applied in a structured manner in order to reason about them.
% To do so it is desirable to apply them to a specific rigorous technique such as a fault trees~\cite{barker1984fault} for safety or attack trees~\cite{schneier1999attack} for security.

Structured graphical reasoning methods help the systematic discovery, assessment and mitigation of risks.
A variety of methods have been used for security and for safety.
% and can be applied to improve the resilience of a system.
While safety usually considers unintentional events and security deals with intentional malicious events,
both safety and security assessments may consider causes and consequences of critical events.
An early method is cause/consequence diagrams~\cite{nielsen1971cause}, commonly
referred to as the ``bowtie method'' due to its graphical representation.
%% DA: text hint since we don't have generic picture
A bowtie is formed of a tree of
causes and a tree of consequences, fanning out to the left and right of a central critical (or \emph{top}) event.
Nodes in the tree represent causal or following events and \emph{barriers} represent ways
to prevent or mitigate events.
Bowties
% This early work allows for the easy observation of causes and consequences and has been used successfully
have been used both for safety~\cite{shahriar2012risk} and security~\cite{bernsmed2017visualizing} separately, and an initial investigation was even performed to inform a safety bowtie by an attack tree~\cite{abdo2018safety} in terms of risk quantification.
They % Bowties
have many desirable properties, such as ease of visualisation~\cite{bernsmed2017visualizing} and the
ability to quantify and calculate likelihoods of events, given a mathematical definition for a diagram's meaning.
%% FIXME DA: is there a canonical citation for that?  Denney?? TO DISCUSS
% , however not all this properties are always used, nor has there ever been an attempt to use them for combined safety security assessments.

In this paper we introduce a way to combine safety and security assessments together in a single
bowtie, to enable reasoning about security and safety together.  In particular we account for four
different types of interplay between event types: safety and security can act independently, with
conditional dependency, in concert, or in opposition ~\cite{kriaa2015survey}.  An ideal structured
reasoning approach should capture each of these.

% Previous work on integrating safety and security interactions have categorised them as
% \emph{independent}, \emph{conditional}, \emph{mut\condition: recent work~\cite{kriaa2015survey} has categorised safety-security interactions as 

% Drawing on the advantages of bowties for reasoning about disruptions and their outcomes we extend standard bowtie definitions to consider the interplay of safety and security.

\paragraph{2021 Facebook DNS outage.} We use Facebook's recent global DNS outage as a running example,
which nicely demonstrates some safety-security interplay~\cite{janardhan2021first,janardhan2021second}. 
On October 4$^{\text{th}}$ 2021, there was a complete outage of all Facebook apps and services (including WhatsApp, messenger, Instagram, etc.), which lasted approximately 6 hours. 
An initial small change to the DNS configuration triggered a complicated chain of events that made resolving a seemingly small issue overly complex and time consuming, and affected millions of people. % & businesses
This happened directly as an outcome of a security response disabling the ability for the safety engineers to patch the server remotely, forcing them to physically access the servers, which exacerbated the disruption.


\begin{figure} [htbp!]
    \centering
    \includegraphics[width=\textwidth]{figs/case-study-fb-leaf.pdf}
    \caption{High level bowtie diagram of the Facebook DNS outage (Tab.~\ref{tab:edge-labels} expands the labels). The negative outcome is in black, whilst the grey path highlights the path that would avoid the negative outcome. Showing the antagonism between the security and safety responses.}
    \label{fig:antagonistic}
\end{figure}

A bowtie describing the sequence of events is presented in Fig.~\ref{fig:antagonistic}.
In outline it shows that the DNS server-down event (the top event) could have a security cause
or a safety cause.  For example, a safety cause could be that a faulty update to the server
configuration goes wrong; a barrier to stop this would be to check the patch doesn't cause
the server to fail.  A security cause might be that an attacker manages to access the DNS
server and make a malicious update.  If the DNS server does go down, we would like to find a path to a
rapid fix to make the server operational again.  But two fixes, a safety
fix and a security fix, are \emph{antagonistic} and act in opposition; only one of them
should be undertaken.  In the Facebook DNS incident, both fixes were implemented,
disallowing remote access to the servers and delaying the response.
% DA: said above forcing engineers to access the server rooms physically.

Obviously this bowtie is not a complete safety-security
assessment (and was constructed after-the-fact).  A more complete model
could cover the many bad consequences that can occur from a central
DNS outage and ways those could be mitigated, as well as further ways
such outages could occur.  But this example serves to demonstrate
how we can model some safety-security interdependences and we will give
mathematical definitions which formalise this, returning to the example
and variations of it in Sec.~\ref{sec:dependencies}.
%% DA: TODO - add mention of the other interplays considered and how
%% we show these with variations of the picture above (right?) LA: yes

%% Can we show TWO OUTCOMES in overall figure
%%
%% 1. What happened - Global DNS outage
%% 2. What should have happened - Temporary/Short downtime
%% 
%%
%% Disruption  = Attack | Fault
%% Prevention  = Barrier | Defence
%% Recovery  OK to use same term already Bowties use Recovery + Mitigation
%% in Event Tree.
%%
%%
%%   Prevention Assessment         &      Recovery Assessment
%%
%%   Disruption Prevention Tree         Disruption Recovery Tree
%% 
%%  Also can we put CAUSES and OUTCOMES labels on left & right
%% 

% Antagonism is present in the safety security measures so that if a security fix is applied, the safety disruption can no longer be patched. This scenario took place in the Facebook DNS incident, disallowing remote access to the servers and delaying the response, forcing engineers to access the server rooms physically

\paragraph{Outline.} The rest of the paper is structured as follows: Sec.~\ref{sec:background} contains background on diagrammatic representation of bowties, we note that further background is added as needed to the respective sections, Sec.~\ref{sec:formalisation} the formalisations of safety-security bowties, Sec.~\ref{sec:dependencies} the interdependence analysis and the formalisation of its operations,  and in Sec.~\ref{sec:conclusions} we provide examples of related work, related assessment techniques, and discuss next steps for this work.



\paragraph{Contributions.} The contributions of this work are the following:
\begin{enumerate}
\item A demonstration of security and safety interplay using bowtie diagrams and
  the Facebook DNS outage.  % This case study provides crucial evidence of the advantages of a unified safety security assessment with
  Fig.~\ref{fig:antagonistic} highlights the need to treat safety and security together, 
  before a critical event and afterwards.
  % clearly showcasing the need for a unified formalisation.
\item Expanding on recent work on combining and formalising safety-security trees as
  \emph{disruption trees}~\cite{stoelinga2021marriage}, we add barriers (safety) and
  mitigations (security), modelling both response forms in  the same formalism.
\item We also add a corresponding mechanism for outcomes, to give a
  new definition for safety-security bowtie diagrams.  %
  %\emph{disruption outcome
  %  trees}.  %% DA: fix name/terminology for RHS
  This provides a solid underlying basis for the graphical notation,
  paving the way for further theoretical analysis and discussion, and
  ultimately towards trustworthy tools to reason about and manipulate such diagrams.
  % repeats above
  % Our work shows that for an accurate interdependence assessment, bowties are crucial to capture the full range of scenarios.
    % \item formalisation of combined safety security outcomes using event trees (right hand side of bowtie diagrams).
\end{enumerate}
This paper is a first step and we want to investigate more complex
case studies as well as studying properties of the definitions,
see Sec.~\ref{sec:conclusions} for more discussion of next steps.




% \textit{Running Example :} Throughout this paper we will be utilising the October 4$^{\text{th}}$ Facebook outage as our running example. With a full assessment presented in Sec.~\ref{sec:case-study}. We showcase the chain of events that lead to the outage and its consequences using CPERO bowties. We also discuss the interplay between the safety and security measures and how they impacted the outcomes of the scenario. As main point of reference we use the reported chain of events by Facebook engineering~\footnote{Initial Update Available at: \url{https://engineering.fb.com/2021/10/04/networking-traffic/outage/}}~\footnote{ Detailed Update Available at:  \url{https://engineering.fb.com/2021/10/05/networking-traffic/outage-details/}} as well as the external assessment conducted by CloudFlare~\footnote{ClaudFlare assessment available at: \url{https://blog.cloudflare.com/october-2021-facebook-outage/}}


% Why it is important to do them together

% Advantages of formal approaches

% Contributions



==> texts/operations.tex <==
\section{Operations for Combinations of Safety Security Assessments}
\label{sec:operations}

%Following from our analysis of safety security interplays in the server outage scenario 
We now formally present notation for how these interplays can be merged into the single assessment.
Different interpretations of how these dependencies are analysed and constructed may exist, depending on model choice and semantics we simply propose operations for the current formalisations and resolve to run a more generic analysis in future works.


\subsection{Independence}

Independence is modelled as two DDTs joining roots with an \texttt{OR} gate.

\begin{definition}
An independent joining of  a security and a safety assessment (assuming both are modelled as disruption defence trees) is defined as: given two disruption defence trees $DDT_{A}$ and $DDT_{F}$ a new tree $DDT_{AF}$ is formed as:
\begin{itemize}
    % \item $DDT_{AF}$ has a unique root, denoted by $RT_{ind}:\neg\exists\  RT_{ind}\  \in N_{AF}\ .\ \forall v \in N_{AF} . RT_{ind} \not\in ch(v)$
    % \item  $RT_{ind}\  \in N_{AF} \ . \ t:RT_{ind} \rightarrow \text{\texttt{OR}}$
    % \item Given the previous vertices of $DDT_{att}$ and $DT_{fault}$, $RT_{att}$ and $RT_{saf}$, the children of  will be $ch:RT_{ind} \rightarrow (RT_{att},RT_{saf})$
    \item $DDT_{AF} := (N_A \uplus N_E \uplus \{R_{AF}\}),\ t_a \uplus t_f \uplus \{\{R_{AF}\rightarrow \text{\texttt{OR}}\},\  ch:R_{AF} \rightarrow (R_{A},R_{F})$
\end{itemize}
\label{def:ind}

\end{definition}



\subsection{Conditional}

A conditional dependence may be viewed as the expansion of a previously unknown external event.
Whilst previously we had a \texttt{LEAF} node that represented an input to an assessment, we now expand this node into a fully fledged disruption tree.
This notion of external event is seen in previous literature~\cite{vesely1981fault}, and this can be seen as an enhancement of knowledge of what lead to the input events.
Semantically it means that a node at the bottom of a disruption tree simply gains as children all the nodes in another disruption tree.

\begin{definition}
A conditional joining of  a security and a safety assessment (assuming both are modelled as a disruption defence tree) is defined as: given a joining of two disruption defence trees $DDT_{A}$ to $DDT_{F}$ a new tree $DDT_{AF}$ is formed as:
\begin{itemize}
    % \item $DDT_{AF}$ has a unique root, denoted by $RT_{fault}$
    % \item for a given final node in $n \in RT_{fault}$ where $\forall\ i\ \in ch:n \rightarrow (\text{\texttt{LEAF}})$ the joining will result in $ch:n' \rightarrow ch:n \cup N_{sec}$
    \item  $DDT_{AF} := \text{if}\ c = t_f(ch:n_F) \rightarrow \{\text{\texttt{LEAF}}\}\ \wedge \ c \sqcap R_A <> \epsilon \implies n_f \uplus R_A, N_A \uplus N_f, ch:n_F \rightarrow \{R_A\}\ \text{else}\ \epsilon$
\end{itemize}
\end{definition}

% \textcolor{red}{Comment: maybe its not a union but rather a replacement, if we include identity function whereby output of tree is labelled then union makes more sense, replacing LEAF with the intermediate event, but semantically doesn't make much difference (I think)}
% \subsubsection{Conditional Example}


% \subsubsection{Antagonistic Example}

\subsection{Reinforcing}

Reinforcing dependence assumes that as an outcome of fixing a fault or mitigating an attack, another fault or attack is no longer possible.
This, in practice, negates a disruption in the disruption defence tree which is being reinforced, which may in some cases make it so that a risk event is no longer possible, as per our case study (see Sec.~\ref{sec:reinforce}).
% For the sake of maintaining the semantics, which allows for much more flexibility and modularity, there is no joining of the tree's but rather an analysis that leads to the alteration of the reinforced tree.
% More specifically if a recovery event is present in the event tree that fixes a fault or mitigates an attack event in the disruption tree, than that event is set as negated for the tree.
As discussed previously, reinforcing dependencies require outcomes/responses to be expressed (right hand side of a bowtie).
The approach taken in this scenario is to transform the whole of the bowtie, into a disruption defence tree joining into the reinforced DDT.
This leads to the final risk event of the reinforced DDT being the new risk event of focus.
We make the assumption that if an event does not lead to any other disruptions in the DDT being reinforced it is not influencing the disruption, and consequently it is negligible and can be pruned (to preserver the tree structure and avoid back propagating branches). We infer that if an event is present in both trees there is an implied relationship, extensions could instead assign further labels to construct these relationships.

\begin{definition}
A reinforcing joining of a disruption recovery assessment (implicitly joining any left most side $DPT$ if a bowtie) $DRA$ and any disruption defence tree $DPT$ takes the form of a joining of the single reinforcing branch by which if a recovery event is present for a fault or attack in $DPT$ that input is negated.
\begin{itemize}
    %\item for $N \in DPT$ and $E \in  DRA$ if $\exists(i . ch:N \rightarrow \{\text{\texttt{LEAF}}\})\in E)$ then $i' = \neg i$
    \item  $DPT_{AF} := \text{if}\ c = t_f(ch:n_F) \rightarrow \{\text{\texttt{LEAF}}\}\ \wedge \ c \sqcap V_A <> \epsilon \implies n_f \uplus V_A, ch:n_F \rightarrow \{\{\text{\texttt{AND}}\} \rightarrow \{\neg c, \{V_A\}\}\} $
\end{itemize}
\end{definition}

We note that an inherent relationship between prevention and disruptions is assumed. 
This is not automatically inferred through formalisations but instead requires expert understanding of the system.
We note under this formalism some knowledge about the events are lost, as they are pruned in the joining.
For clarity, an example joining between $DRA_i$ and $DPT_j$:
\begin{equation*}
    DRA_i = (\text{\texttt{X}} \cap \text{\texttt{Y}}) \ \text{and}\ DPT_j = ([j_i\cap \overline{j_i},j_n \cap \overline{j_n}])
\end{equation*}
if $j_n$ is equals to $X$, their antagonistic joining $DRA_{ij}$, joins the path $V_j =\{j_i,j_n\}$ to $DPT_i$
\begin{equation*}
    DRA_{ij} = ((\neg\text{\texttt{X}}\cap V_j ))\cap \text{\texttt{Y}})
\end{equation*}
We note this representation of a path of potentially several actions may be seen as a hierarchical label, whereby a path to an event is simply boxed to represent a single event.


\subsection{Antagonistic}

Antagonistic relationship mean that a security outcome, such as a repair, makes it so that a safety outcome cannot take place. 
In practice this means that the system can either be made safe or it can be made secure, but not both.
This unlike the previous relationships is modelled through the recovery assessment and through the usage of event trees.


\begin{definition}
A antagonistic joining of  a security and a safety recovery is defined as: given a joining of two disruption recovery assessments  $DRA_{A}$ and $DRA_{F}$ a new tree $DRA_{AF}$ is formed as:
\begin{itemize}
    % \item $E_{AF} \in DRA_{AF}$ is given by a union between $E_{att} \in DRA_{att}$ and $E_{fault} \in DRA_{fault}$
    % \item given antagonistic event $a_e \in E_{AF}$ caused by $a_e = (e_{sec} \in E_{att}) \cup \Bar{ (e_{saf} \in E_{saf})}$ the next state $s+1 \in S_{AF}$ the branching will be calculated as $a_e$ and $\Bar{a_e}$
    % \item $a_e$ and $\Bar{a_e}$ determines that either $e_{sec}$ can take place but not $e_{saf}$ or conversely.
    \item $DRA_{AF} := E_A \uplus E_S, e_a = e_s \in E_{AF} \implies S_{AF}+1(e_a,e_s) \rightarrow e_a \oplus e_s$
\end{itemize}
\label{def:antagonistic}
\end{definition}



\subsection{Formalisation of Facebook DNS Disruption as a Bowtie}

Following from the described notation, using \texttt{AND}($\cap$), \texttt{OR}($\cup$) and \texttt{INHIBIT}($\hexagon$), we can define the bowtie displayed graphically in Fig.~\ref{fig:antagonistic} in the following steps:

\noindent given the safety scenario $DPT_S$:
\begin{equation*}
    DPT_S = ((\text{\texttt{server patch}}\ \hexagon\ \text{\texttt{update check}})\cap(\text{\texttt{resolve DNS}}\ \hexagon\ \text{\texttt{dns check}})) 
\end{equation*}
\noindent and given the attack scenario $DDT_A$:

\begin{equation*}
    DPT_A = ( ((\text{\texttt{ftp}}\ \cap\ \text{\texttt{rsh}})\ \cap\ \text{\texttt{buffer overflow}})\ \cup\ (\text{\texttt{rsa}}\ \cap\ \text{\texttt{ssh}})
\end{equation*}
\noindent they can be \textit{independently} joined following Def.~\ref{def:ind} to form:
\begin{equation*}
\begin{split}
 FB_{DPT} = &  ( ((\text{\texttt{ftp}}\ \cap\ \text{\texttt{rsa}})\ \cap\ \text{\texttt{buffer overflow}})\ \cup\ (\text{\texttt{rsa}}\ \cap\ \text{\texttt{ssh}}))\ \ \cup \\
 & ((\text{\texttt{server patch}}\ \hexagon\ \text{\texttt{update check}})\cap(\text{\texttt{resolve DNS}}\ \hexagon\ \text{\texttt{dns check}})) 
 \end{split}
\end{equation*}
\noindent and then given the two possible consequence trees, ${[DCT_A,DCT_S]}$:
\begin{equation*}
   DCT_S = (\text{\texttt{remote login}})\ \text{and}\ DCT_A=(\text{\texttt{disable ssh}})
\end{equation*}
\noindent we can antagonistically join them following Def.~\ref{def:antagonistic} to form the FB case study situation of conflict:
\begin{equation*}
\begin{split}
FB_{DCT} = & (\text{\texttt{remote login}}\ \cap\ \overline{\text{\texttt{disable ssh}}})\ \cap\ (\overline{\text{\texttt{remote login}}}\ \cap\ \text{\texttt{disable ssh}}) \\
& \text{ or more simply }(\text{\texttt{remote login}}\ \oplus\ \text{\texttt{disable ssh}}). 
 \end{split}
\end{equation*}
Putting the two together you can obtain the bowtie $FB_{Bowtie} = [FB_{DPT} \rightarrow [[\text{\texttt{server outage}} ]] \rightarrow FB_{DCT}]$


==> texts/related-work.tex <==
This work is by no means the first exploration of combining security and safety~\cite{gould2020safety,kriaa2015survey,kriaa2014safety,abdo2018safety,haider2019concertofla}.
Existing work in the area also highlights that this is by no means an easy feat as there are several differences as an outcome of developing in completely different contexts~\cite{gould2020safety}.
Gould and Bieder~\cite{gould2020safety} explore the initial development of the two fields and the contexts in which they coexist.
Safety is originally developed as means to avoid systems failures guided by the increased understanding of hazards and inevitability of accidents.
Conversely, security developed initially as an outcome of malicious parties wishing to harm systems, however has developed into a critical component of any system analysis.
The authors cite the increase of emphasis on the reduction of risks associated with mitigating security threats as a key factor as to why security and safety should be integrated more.
However security and safety fields diverge vastly on technology usages and quantification of risks.
The two fields however are strongly interconnected and as such their integration is essential.
The authors propose the need for new policies and shared practice as without the other neither field can be complete and neither safe nor secure~\cite{gould2020safety}.
This recent work highlights the need to unify the assessment techniques, although they do not provide intuition as to how to do so.
Literature has already considered how these two fields may be considered under the same methodology~\cite{haider2019concertofla}, however, often this is done rather relying on expert analysis and without underlying formal foundations.
However, there have also been some specific assessment techniques proposed to join the two assessments.

\subsection{Assessment Techniques}

An emerging field that has a deep integration between these two topics is that of industrial control systems (ICS)~\cite{kriaa2015survey}.
Industrial systems have always been focused on safety, however with the new integration of internet infrastructure and the IoT the avenues of attack greatly increase~\cite{arnaboldi2020modelling,arnaboldi2017quantitative}, leading to the need for better security evaluations to be in place.
Work by Kriaa et al.~\cite{kriaa2015survey}, surveys a list of techniques used in this field for both safety and security.
In this work the authors discuss the possibility for a safety case to be broken by security threats and discuss means to address this in the system assessment.
% The authors extend previous work on the subject~\cite{eames1999integration}, to categorize the relationships in the following four manners: 1) \textit{conditional dependency}, 2) \textit{mutual reinforcement}, 3) \textit{antagonistic}, and 4) \textit{independence}.
The paper also discusses current standards for safety and security in the context of ICS, how they may integrate and assessments to decide which category needs to be considered.
Using a different formalism of BMDPs previous work has similarly used the case study of a pipeline to observe security and safety interactions~\cite{kriaa2014safety}.
Their work was one of the first to evaluate the different interdependency types. 
In more recent work~\cite{gallina2022multiconcern} address this same topic in the context of safety and security assurance.
In this work the authors conduct an hazard analysis and risk assessment (HARA) a common safety assurance methodology alongside a threat analysis and risk assessment (TARA), which can be used to assess security risks.
Combining these two techniques they are able to conduct a unified safety security assessment for their case study of an autonomous vehicle adhering to the safety standard ISO26262 and security standard ISO21434 for autonomous vehicles.
Although we note that the unification of these techniques is not done formally under a single construct but more as an iterative manual process.


% Integrating Formal Verification and Assurance:An Inspection Rover Case Study~\cite{bourbouh2021integrating}
Having established the need for rigourous security assessment recent work experimented with the usage of bowties for this purpose~\cite{bernsmed2017visualizing}.
In their work the authors apply the usage of bowties to security analysis in the maritime industry.
They showcase the flexibility of the approach in quantified various threats and calculating the impact of the attacks. 
The paper proposes a formula for quantifying threat and consequence impact.
The authors also ran a user study showed that people in the maritime industry thought Bowties for security were a very useful tool, showcasing the applicability of bowties to industry case studies.
The first approach combining safety and security bowties~\cite{abdo2018safety}, combines an attack tree with a safety bowtie, and whilst this proves to be a great first step, falls short of completely uniting the various interdependencies into a single assessment.
%which can easily be added in (and needs to be expanded upon to fit our formalisation). Their survey s

The literature showcases that there is already a wide use of these techniques across a wide range of fields and a formal representation allows to set the foundations for further expansions and reasoning.
Formal descriptions allow to have a more rigorous way to analyse systems, they allow to establish what you can and can't do using the approach as well as reason about properties of a formalism.
Previous work has applied this in the context of safety cases~\cite{denney2015formal} and showcased it as a valuable way to create and assess system evaluations.
Even more so, security researchers have applied formal representations to attack trees~\cite{jhawar2015attack,mauw2005foundations}, showcasing its usefulness to reason about systems and performing structured analysis~\cite{fila2020exploiting}.
In more recent work~\cite{denney2019role} the authors formalise bowties in and causality sequences for usage of safety and avionics, their formalisation is similar to the one used in this work, although they omit the analysis of interdependency.
As such they do not discuss joining operations and do not assess security and safety under the same construct, which lies at the foundation of our security and safety assessments.
% What is still missing from the literature is the formalisation of how exactly the interdependence of these two fields impacts an assessment and how these can be combined in a structured manner to conduct a single (and very needed) unified assessment.
Our work begins to apply the same formal rigour to safety and security assessments using bowties to unify the assessment in a structured and formal manner, both drawing from clear semantic understanding as well as a clear visual representation.




